Explaining in Style: Training a GAN to explain a classifier in StyleSpace

Image classification models can depend on multiple different semantic attributes of the image. An explanation of the decision of the classifier needs to both discover and visualize these properties. Here we present StylEx, a method for doing this, by training a generative model to specifically explain multiple attributes that underlie classifier decisions. A natural source for such attributes is the StyleSpace of StyleGAN, which is known to generate semantically meaningful dimensions in the image. However, because standard GAN training is not dependent on the classifier, it may not represent these attributes which are important for the classifier decision, and the dimensions of StyleSpace may represent irrelevant attributes. To overcome this, we propose a training procedure for a StyleGAN, which incorporates the classifier model, in order to learn a classifier-specific StyleSpace. Explanatory attributes are then selected from this space. These can be used to visualize the effect of changing multiple attributes per image, thus providing image-specific explanations. We apply StylEx to multiple domains, including animals, leaves, faces and retinal images. For these, we show how an image can be modified in different ways to change its classifier output. Our results show that the method finds attributes that align well with semantic ones, generate meaningful image-specific explanations, and are human-interpretable as measured in user-studies.

==> fig_diversity.tex <==
\begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{figures/diversity.png}
   \vspace{-.2in}
   \caption{{\bf Explanations diversity}.
   Each path is a disjoint set of two attributes that, when applied to the original image on the left, changes the classification result.}
   \label{fig:diversity}
\end{figure}

==> rebuttal/contents.tex <==

\noindent We thank the reviewers for their valuable comments. We appreciate the reviewers' recognition of the novelty in our contribution, and hope that this paper will motivate follow-up work on counterfactual attribute-based explanations.

\R{R1:} We thank the reviewer for the positive review and for pointing out grammatical errors. These errors will be fixed.

\R{R2: Evidence for actual impact of the work}
\reviewer{There are no experiments that demonstrate the actual impact of the work. Results do not show that medical practitioners find the attributes intuitive and useful.}
	
For results on the Retina dataset, we consulted with an expert ophthalmologist who confirmed that 3 of the 4 attributes are known attributes; we refer to this in the caption (lines 577-578), but will further clarify. Furthermore, the ophthalmologist provided a reference describing the recognized attributes, please see \textbf{(add reference here)}.

\R{R2: Comparison to other methods in terms of visual quality and usefulness}

\reviewer{It is hard to believe there are no other relevant methods to compare to, beyond Wu. StarGAN and the variety of other papers that modify attributes come to mind-- these don't modify attributes relevant to classifier outputs, but could be compared to from a visual quality point of view. Further, given the large number of interpretability/explainability papers, how about comparing some of those to the proposed, in terms of how useful the visualization results are for a practitioner or anyone trying to understand classifier outputs?}

The goal of our method is to explain a classifier by identifying attributes relevant to classifier predictions, rather than to produce image manipulations of high visual quality. StarGAN, as the reviewer mentions, does not modify attributes relevant to classifier outputs, and furthermore our attributes are extracted in an unsupervised manner (i.e. they are not aligned with any labels that may be provided to StarGAN during training). It is therefore unclear to us how to compare our main contributions to StarGAN. We will be happy to take suggestions from the reviewer. As for other interpretability papers, Fig. ~2. gives an example of why generative models can be more useful than heatmaps (e.g. it is unclear how to visualize the absence of ``spots" with a heatmap), it is easy to imagine how this extends to medical examples. Other interpretability papers that manipulate attributes with generative models, either use labelled attributes or only work on small scale datasets. We will further clarify this in Sec. ~2.

For the first part, I think we can say that the paper does not claim new methods for attribute manipulation and that in fact we directly cite the stylespace paper, therefore we don’t need to compare visual quality.
For the second part, we can say that in section 2 we discussed the many other explainability methods and why we can’t compare to them, but that we could clarify it better in the final version
But if there other ideas for comparison it could be better, let’s discuss
Just another small note here: It might be useful to stress that since our attributes are extracted in an unsupervised manner, a comparison with StarGAN is vacuous (given an attribute that we extracted, which StarGAN should we compare it to?).


\textcolor{blue}{Fig. 5 includes zoom-ins-- but the method doesn't output these. If zoom-ins are important, who will select these in an automated setting?}

The zoom-ins were meant to highlight things in a static figure in the paper; they are clearly visible in a dynamic video (which is the mode of our explanation), and are not necessary there.
We could show the image diff between these images and explain how we could zoom in to the area with the maximal diff. 
Additionally we could point to the supplementary material where the differences are much clearer without the need for zoom-ins

\textcolor{blue}{The importance of disentangled attributes doesn't seem to be quantitatively demonstrated.}

Long term goal is to quantify with downstream applications, such as how well this helps doctor’s make decisions. Demonstrating clinical use is an important next step but our paper focuses on the first step of showing a qualitatively new method: showing multiple attributes that separately affect a classifiers output.


I am not sure how to respond to this one. I don’t think we need quantitative demonstrations for this, no?
\textcolor{blue}{Additional comments}


\textcolor{blue}{Some intuitions/motivations are repeated many times, which is not necessary.}
I also felt it too, we could maybe remove some in the later sections

\textcolor{blue}{In Table 3, the difference between methods is very different on difference datasets, e.g. 83-83 vs 18-66 for Ours w/o CST vs Ours-- why might that be?}
I think we addressed this specifically in lines 843-850

\textbf{Reviewer 3:} Weaknesses
\textcolor{blue}{One major concern of the reviewer emerges from Fig. 4 in the paper. Firstly, the reviewer does not find the tasks "perceived gender" or "perceived age" classification is ethically well motivated. The authors may provide a justification of why perceiving gender or age are scientifically interesting and ethically appropriate as computer vision tasks.}

The goal of our method is not to explain age or gender, but rather to explain what classifiers are learning, and their biases (hence the word “perceived”). We believe that understanding what has led a classifier to reach its decision is a very important research topic in CV research. We think it is especially important to explain face analysis systems due to the social implications of their real world usage. Our method can reveal potential biases in these systems as we emphasized on line … We will further clarify in the figure captions that the attributes we are visualizing are an explanation of the classifier and not a claim that these are the true attributes that determine age or gender. Prior work on explaining gender bias in classifiers has been influential toward creating fairer and more accurate systems (Gender Shades, work from Lisa Anne Hendricks, etc). We very much agree with the reviewer about the sensitivity and importance of this topic and will add greater discussion in the paper so that our results are not misinterpreted.


We need to stress out that the purpose of this demonstration is not to study the attributes of perceived gender or age, but rather study the attributes of classifiers trying to do it, and expose their biases. We talk about it briefly in the conclusion but apparently not enough.
One experiment that we could add, and indeed started doing before the paper but didn’t have enough time, is comparing gender / age classifiers from different networks and different datasets. For example comparing biases of ResNet to biases of MobileNet, and comparing biases of models trained on Celeb-A to ones trained on FFHQ. [michaly: I also did an experiment on dogs/cats dataset, I compared two classifiers and got different results - I can try to reproduce it if it will be useful].

\textcolor{blue}{Furthermore, what is also concerning is that the attributes being discovered essentially may correspond to biases in the dataset. For instance, "eyeglass lenses" or "mouth open/close" should not have any impact on age classification. In the case of "perceived gender classification", the reviewer is not convinced if lipstick and eyebrow thickness are relevant attributes. While the authors do mention that this method can be useful in uncovering and mitigating bias in classifiers (line 100 and line 858), there is no other mention that this problem exists even when it's clearly evident in the figure (and in the supplementary material). It would be re-assuring if the authors explicitly discussed this issue either while discussing the qualitative results or having a broader impact section which discusses this issue.}


Once again, our method aims to explain what the classifier has learned (along with its biases -- some of them potentially due to dataset bias). Our method does not claim to explain reality.


I think we can fully agree to this comment, and say that it actually demonstrates the strength of the method, which is exposing exactly those biases. On retrospect we should have included this discussion in the relevant section.

\textcolor{blue}{Finally, it appears that the classifiers have been used primarily for binary classification (apart from the cat species, but that has not been illustrated). It would be helpful if the authors were able to either provide results for multi-class classification problems or if that is not possible, it would be useful if the authors can provide some explanation regarding the challenges in performing such an experiment. This is especially interesting because this method would be most useful in fine-grained classification problems (eg. CUB) where the difference between classes can be explained entirely with attributes. Whereas, in a coarse-grained classification tasks such as cats vs dog (from Fig. 1), the attributes do not seem to be the deciding factor in the classification (eye/ear shape, or open/close mouth). Therefore, even after altering these attributes, the decision should remain the same, which is indeed the case in Fig. 1, even if the likelihood of the prediction changes.}

Regarding multiclass - we could show some results from the wild cats classification, and describe the change in the AttFine algorithm we used to find them.
Regarding the CUB dataset - I disagree with the reviewer here, I think the fine grained classification will be quite trivial and each S will correspond to a single class. I might be wrong here though, we could try and run an experiment there. Another option is to run experiment on the fine-grained plants classification (38 classes), but if I remember correctly the results of this experiment were not too good.
It is true that for cats/dogs we need much more attributes than other domains, but in most other domains we needed very few attributes.


\textcolor{blue}{Additional comments}
\textcolor{blue}{Broader impact:
The reviewer believes that this work can set off a new line of counterfactual methods for explainability, which would be very useful. In addition, this work could be an important tool in covering the biases inherently present in many classification models as well as in datasets (see the discussion paragraph 2 in weaknesses).}
Very good point for us I think

\textcolor{blue}{Comparison with the state of the art:
The reviewer is not aware of any other method that solves the same problem. Therefore, it is understandable that the authors did not have an exact competitor to be reported in the results. However, when compared to other popular methods used for explainability, it is clearly different and demonstrates its benefits. Additionally, there is an ablation study which demonstrates the benefit of the classifier-specific training as well.}
Again, a very good point for us.

\textcolor{blue}{Reproducibility:
The authors do not indicate if they will release the code once the paper is accepted. If the code is not released, making a comparison with this work in future would be quite tricky since a lot of implementation details mentioned in the paper, e.g. "the classifiers are based on the MobileNet [12] architecture, and achieve a high accuracy of at least 95\% on their test sets", is not enough to reproduce the results. So the combination of being unclear about the implementation details, missing dataset statistics and not having access to the code could be a problem for reproducibility.}
Hmm… This is true… We discussed this in the past, it’s difficult to release all the necessary things for this method to be reproducible because we would need to release both the classifiers and the GANs, which is problematic and difficult. But maybe there are things we could release.

\textcolor{blue}{Other Comments:
One perspective that the authors might want to think about is the connection with black-box adversarial attacks. For instance SimBA (https://arxiv.org/abs/1905.07121) performs a greedy search over the pixel space and attempts to perturb pixels that maximize the change in the classifier prediction. This is very similar to the "Subset" strategy proposed here, the difference being that the changes are done in the StyleSpace and then generated using a GAN instead of directly modifying the pixel space.}
This exact difference, the fact we search style-space and not pixels, is what makes our method non-adversarial. Adversarial attacks are interesting in their own aspect, but they do not contribute to explainability.
IMHO it sounds like we should respond along the lines of “thanks, we will add a reference in the related work section”.

\textcolor{blue}{It would have been helpful if the authors provided a supplementary material which discussed the datasets and how they were used in a bit more detail. For instance, for the age classification, the reviewer couldn't find the age annotations in the FFHQ dataset so the reviewer is not sure sure how exactly it was converted into a binary classification problem. The reviewer understands that the authors did not have space in the main PDF and therefore only have a table mentioning the dataset and the task, but providing a bit more detail in the rebuttal would be useful.}
We did not want to get into it in the paper, but it looks like we are going to have to address this. 

\textcolor{blue}{
The reviewer encourages the reviewers to provide a discussion about all the points raised in the 'weaknesses' as well as in the 'detailed comments' in the rebuttal.}


==> rebuttal/fig_multi_class_cub.tex <==
% \begin{figure}[b]
   \includegraphics[width=0.98\columnwidth,scale=0.9]{LaTeX/figures/CUB-one-vs-all.pdf}
%   \label{fig:multi_class}
% \end{figure}
